Object Detection in Aerial Images in Scarce Data Regimes

Most contributions on Few-Shot Object Detection (FSOD) evaluate their methods on natural images only, yet the transferability of the announced performance is not guaranteed for applications on other kinds of images. We demonstrate this with an in-depth analysis of existing FSOD methods on aerial images and observed a large performance gap compared to natural images. Small objects, more numerous in aerial images, are the cause for the apparent performance gap between natural and aerial images. As a consequence, we improve FSOD performance on small objects with a carefully designed attention mechanism. In addition, we also propose a scale-adaptive box similarity criterion, that improves the training and evaluation of FSOD methods, particularly for small objects. We also contribute to generic FSOD with two distinct approaches based on metric learning and fine-tuning. Impressive results are achieved with the fine-tuning method, which encourages tackling more complex scenarios such as Cross-Domain FSOD. We conduct preliminary experiments in this direction and obtain promising results. Finally, we address the deployment of the detection models inside COSE's systems. Detection must be done in real-time in extremely large images (more than 100 megapixels), with limited computation power. Leveraging existing optimization tools such as TensorRT, we successfully tackle this engineering challenge.

==> chapters/acknowledgement.tex <==
\makeatletter
\let\savedchap\@makeschapterhead
\def\@makeschapterhead{\vspace*{-9em}\savedchap}
\chapter*{Remerciements}
\let\@makeschapterhead\savedchap
\makeatletter
\vspace{-3em}
\addcontentsline{toc}{chapter}{Remerciements} 

Je tiens tout d'abord à remercier ma directrice de thèse Anissa MOKRAOUI,
Professeur à l'Université Sorbonne Paris Nord, pour son encadrement, son
soutien, ses conseils avisés et sa disponibilité tout au long de cette thèse. 

Je remercie également Hervé GUIOT et Olivier GUITTON de l'entreprise COSE qui
ont suivi et supervisé ce projet avec attention. J'en profite pour remercier
COSE de manière générale pour le financement de cette thèse. Il me faut
également écrire un mot pour mes collègues dans l'entreprise qui m'ont apporté
un soutien moral quotidien pendant ces trois ans. En particulier, merci à
Brice, Chloé, François, Kimmeng, Lotfi, Maxime, Remi et Ugo. 

Merci à l'ensemble des membres du jury de ma thèse d'avoir accepté
d'évaluer mes travaux de recherche et d'avoir formulé des remarques
constructives pour l'amélioration de ce manuscrit.  

Je voudrais ensuite remercier Damien, Florian, Jules, Quentin, Tanguy et Thibaut
pour leurs relectures attentives et leurs questions pertinentes qui m'ont
grandement aidé dans la rédaction de ce manuscrit de thèse. Merci aussi pour
les moments de détente passés avec vous au cours des trois dernières années qui
m'ont permis de décompresser quand cela était nécessaire. 
%
% J'exprime ma gratitude envers l'ensemble des personnes qui ont pris le temps de
% répondre à mon étude sur la perception humaine de la qualité des détections
% d'objets. Les données ainsi collectées ont donné lieu à une publication.  

Ensuite, je voudrais remercier Hicham TALAOUBRID et Lièce CHERCHOUR, stagiaires
chez COSE qui ont été d'une grande aide dans l'obtention de certains résultats,
l'implémentation et le déploiement de plusieurs algorithmes.  

Je remercie aussi l'ANRT pour le financement de cette thèse, le L2TI et le
LabCom IRISER (ANR-21-LCV3-0004) pour leur cadre scientifique, et enfin le GENCI
pour la mise à disposition de moyens de calcul de l'IDRIS au travers de
l'allocation de ressources 2022-AD011013955.

Merci également à MM. BROUARD et VILQUIN, enseignants au Lycée Sivard de Beaulieu
de Carentan, ils m'ont initié aux Mathématiques, à la Physique et à l'Informatique.
C'est grâce à eux que j'ai cette passion pour les sciences.

Je dois aussi remercier ma famille, et en particulier ma mère de m'avoir
toujours poussé et soutenu dans mes études. Sans cela, je ne serai certainement
pas là où j'en suis aujourd'hui.  
 
Enfin, je ne peux pas conclure sans remercier Marie du fond de mon cœur. Je te
remercie pour tes nombreuses relectures, mais surtout pour ton soutien
indéfectible au quotidien et tes encouragements souvent indispensables. Sans
toi, je n'y serai pas arrivé ! 

À mon père. 



